GlycanML: A Multi-Task and Multi-Structure Benchmark for Glycan Machine Learning

Glycans are basic biomolecules and perform essential functions within living organisms. The rapid increase of functional glycan data provides a good opportunity for machine learning solutions to glycan understanding. However, there still lacks a standard machine learning benchmark for glycan property and function prediction. In this work, we fill this blank by building a comprehensive benchmark for Glycan Machine Learning (GlycanML). The GlycanML benchmark consists of diverse types of tasks including glycan taxonomy prediction, glycan immunogenicity prediction, glycosylation type prediction, and protein-glycan interaction prediction. Glycans can be represented by both sequences and graphs in GlycanML, which enables us to extensively evaluate sequence-based models and graph neural networks (GNNs) on benchmark tasks. Furthermore, by concurrently performing eight glycan taxonomy prediction tasks, we introduce the GlycanML-MTL testbed for multi-task learning (MTL) algorithms. Also, we evaluate how taxonomy prediction can boost other three function prediction tasks by MTL. Experimental results show the superiority of modeling glycans with multi-relational GNNs, and suitable MTL methods can further boost model performance. We provide all datasets and source codes at https://github.com/GlycanML/GlycanML and maintain a leaderboard at https://GlycanML.github.io/project

==> sections/07_impact.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Broader Societal Impacts} \label{sec:impact}

This work aims at building a comprehensive benchmark for glycan machine learning, incorporating diverse types of glycan understanding tasks, multiple representation methods of glycan structures, and a testbed for multi-task learning algorithms. By evaluating on the proposed benchmark, we can judge the general effectiveness of a machine learning model on predicting different glycan functions. Therefore, such a benchmark can promote the application of machine learning methods to various real-world glycan-related tasks, such as vaccine design~\cite{kaplonek2018improving} and cancer research~\cite{taniguchi2015glycans}. 

However, we should not ignore the potential harmful aspects brought by glycan machine learning models developed on our benchmark, \emph{e.g.}, designing vaccines with severe adverse reactions. To mitigate such risks, our future works will encourage the responsible usage of the \our{} benchmark for real-world problems. 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

